Laws of thermodynamics for exponential families

We develop the laws of thermodynamics in terms of general exponential families. By casting learning (log-loss minimization) problems in max-entropy and statistical mechanics terms, we translate thermodynamics results to learning scenarios. We extend the well-known way in which exponential families characterize thermodynamic and learning equilibria. Basic ideas of work and heat, and advanced concepts of thermodynamic cycles and equipartition of energy, find exact and useful counterparts in AI / statistics terms. These ideas have broad implications for quantifying and addressing distribution shift.

==> experiments.tex <==
\section{Algorithms and experiments with them}

All these quantities are easily computable in principle given $\lambda, f (x), \alpha$, for any exponential family. 
The exponential families we are interested in are learned models like softmax regression, which we are interested in e

Easy to fine-tune by adding a couple more features. Free energy will only decrease, right? Measure this. 


Try heat+work decomposition for a simple example with a logistic regressor where the data changes, and decompose the change in performance of the regressor (change in the free energy) into work and heat. 
We've shown that the score function is determined by the internal energy, and the regret is determined by the free energy. 
Take it through a zero-heat process, all adiabatic, where the regret doesn't change because the energy is conserved. 



the book [@thompson2015mathematical] contains more examples.


